Rethinking Prompting Strategies for Multi-Label Recognition with Partial Annotations

Vision-language models (VLMs) like CLIP have been adapted for Multi-Label Recognition (MLR) with partial annotations by leveraging prompt-learning, where positive and negative prompts are learned for each class to associate their embeddings with class presence or absence in the shared vision-text feature space. While this approach improves MLR performance by relying on VLM priors, we hypothesize that learning negative prompts may be suboptimal, as the datasets used to train VLMs lack image-caption pairs explicitly focusing on class absence. To analyze the impact of positive and negative prompt learning on MLR, we introduce PositiveCoOp and NegativeCoOp, where only one prompt is learned with VLM guidance while the other is replaced by an embedding vector learned directly in the shared feature space without relying on the text encoder. Through empirical analysis, we observe that negative prompts degrade MLR performance, and learning only positive prompts, combined with learned negative embeddings (PositiveCoOp), outperforms dual prompt learning approaches. Moreover, we quantify the performance benefits that prompt-learning offers over a simple vision-features-only baseline, observing that the baseline displays strong performance comparable to dual prompt learning approach (DualCoOp), when the proportion of missing labels is low, while requiring half the training compute and 16 times fewer parameters

==> old_intro.tex <==
%Image recognition is one of the most fundamental task in computer vision, where the goal is to identify the objects within an image. Significant progress in this field has been driven by the availability of large-scale datasets and advanced neural networks. However, 

Multi-label recognition (MLR) has gained increasing attention due to its relevance in real-world applications. Unlike single-label recognition, where an image is associated with just one label, MLR requires identifying multiple objects or concepts present in an image, making it significantly more challenging. Examples of MLR applications include medical diagnosis from chest X-rays \cite{huang2024radiology}, product detection in e-commerce images \cite{ecomm_product}, and food recognition for dietary monitoring systems \cite{nutrient2,nutrient3}.

The complexity of MLR arises from the combinatorial increase in the number of possible label subsets, which escalates the need for annotations. However, obtaining sufficient annotations is often infeasible, especially in the presence of class imbalances or rare classes \cite{rare}. This creates a pressing need to address MLR with limited annotations, which is crucial for improving the recognition performance of  systems in real-world scenarios.


Recently, multiple approaches have emerged to address the challenges posed by limited or missing annotations in MLR. These advances have led to significant performance improvements, with one key factor being the adoption of VLMs such as CLIP. Unlike traditional ImageNet-based initialization \cite{deng2009imagenet}, CLIP's initialization offers a notable advantage due to its training on a much larger and more diverse corpus, resulting in stronger and more generalizable representations. As demonstrated by several VLM based MLR approaches \cite{dualcoop,MLR-CoOp,scpnet}, VLMs not only enhance MLR performance but also is efficient by reducing the number of trainable parameters.

VLMs in MLR has been motivated by the desire to take advantage of the visual and text features in the shared embedding space resulting from the vast amount of VLM training with visual and text inputs. This has indeed boosted the performance of the resulting MLR methods in the limited annotations regime.
The most prominent approach for adapting VLMs for MLR is by learning textual prompts that maximize similarity with image features, a strategy commonly referred to as prompting. DualCoOp \cite{dualcoop} and DualCoOp++\cite{dualcoop++} are two state-of-the-art (SOTA) prompting-based approaches that rely on learning a positive and negative prompts for each class. The positive prompt indicates the presence of a class, while the negative prompt indicates its absence. 
These approaches empirically demonstrate that learning a negative prompt alone significantly reduces performance, even to levels lower than those achieved with handcrafted prompts. While learning a positive prompt yields good performance, the best results are achieved when combining learned positive and negative prompts.
Despite their empirical success, these methods do not provide any analysis of the observed performance hierarchy, leaving several key questions unanswered: (1) Why do learned negative prompts underperform compared to handcrafted prompts, and why do they perform significantly worse than learned positive prompts?  (2)  Given the poor results of learned negative prompts, could they also limit the performance in the joint setup of DualCoOp (learning both positive and negative prompts)? At the core of these questions lies the underperformance of learned negative prompts. We investigate the reasons behind this limitation.

% 
In DualCoOp, the learned positive prompt is $[V^+]\{\text{classname}\}$, and the learned negative prompt is $[V^-]\{\text{classname}\}$, where $V^+$ and $V^-$ are the learned context vectors. The positive prompt $V^+$ enhances similarity between object regions and prompt features, while the negative prompt $V^-$ reduces it. However, negative prompts may not align with CLIP's design because it is primarily trained on positive captions, meaning it is optimized to recognize the presence of objects rather than their absence. For example, when given an image of a car, the caption would describe the car rather than focusing on the non-car regions with phrases like 'Not a photo of a car' or 'absence of a car. Fig. \ref{fig:CLIP's activation} demonstrates that CLIP activates the same regions in the image with positive and a negative prompts. Does this mean that the use of negative prompts reduce the benefits of the latent representation? Should the use of negative prompts as in SOTA methods therefore be replaced with something more effective?

These are the key questions we address in this paper. Specifically, we test the hypothesis that using negative prompts not only \textit{hurts} performance when used individually, as shown in DualCoOp \cite{dualcoop} and DualCoOp++ \cite{dualcoop++}, but also in their joint learning setup(learning positive and negative prompts). If this is the case, how can we improve these methods? To explore this, we first establish a baseline using a simple one-layer MLP applied to visual features, deliberately excluding the text encoder. This baseline enables us to quantify the performance degradation associated with learned negative prompts. 

Next, we investigate their joint learning setup. To address the issues observed with negative prompts, we propose a hybrid setup, Positive CoOp, where we replace the negative prompts with a fixed prompts that are optimized in feature space. Specifically, rather than relying on CLIP to project a learned negative prompt into its embedding space—an operation CLIP was not originally designed for—we use a fixed prompt for each class. This fixed prompt is projected by CLIP, and we augment this projection with learnable features. By doing this, we align with CLIP’s strengths: we leverage the effectiveness of the learned positive prompt, which CLIP handles well, while refining the negative prompt features in the feature space without CLIP. The rest of the setup follows the standard DualCoOp framework for multi-label recognition task.

We evaluate our one-layer MLP baseline and the Positive CoOp setup on two standard multi-label recognition (MLR) benchmark datasets: COCO \cite{coco} and VOC \cite{pascal-voc}. Our results show that the baseline achieves competitive performance compared to DualCoOp, while requiring approximately 12 times fewer training parameters and X times fewer training hours, averaged across the two datasets. Additionally, Positive CoOp surpasses DualCoOp in performance on both datasets, requiring 5 times fewer training parameters and approximately half the training hours, denoted as 
Y, compared to DualCoOp. 


% The results show that even this simple classifier, with only visual features, outperforms all SOTA methods on standard benchmarks like COCO \cite{coco} and VOC2007 \cite{pascal-voc}, while significantly reducing the number of training parameters (5 times on average) and training hours (2 times on average) across the two datasets. Fig \ref{fig:Difference from Existing approaches} provides a high-level comparison of our method with existing MLR approaches.
% To test our hypothesis, we compare the performances of negative prompts based method, our no-prompts baseline, and the case using only positive prompts, and as may be expected from the discussion above, the additional information in positive prompts indeed raises the performance over the baseline case (which is already above the SOTA case of using both prompts). 


% We see our experiments using MLP as being useful for showing the roles of text prompts, as discussed in Sec \ref{Sec:Analysis}. We do not propose this as our solution for MLR with limited annotations, because our experimental linear setup may be enhanced in several ways, such as using visual prompting, text prompting,  prior knowledge from training data or domain adaptation.


% The empirical performance of our approach should not be considered a novel solution for MLR with limited annotations. We believe that several directions, such as visual or textual prompting, prior knowledge from large models, or domain adaptation, would better help the adaptation of VLMs for MLR. However, the effectiveness of our simple setup suggests that certain aspects (Sec \ref{Sec:Analysis}) of the current VLM-based SOTA MLR approaches lead to their sub-optimal performance.


We summarize our contributions as follows: \\
1) We validate and analyze the impact of negative prompts on multi-label recognition performance, demonstrating that their use adversely affects model performance.\\
2) Our hybrid setup, Positive CoOp show that joint learning methods \cite{dualcoop, dualcoop++}is suboptimal due to the learning of negative prompts. In contrast, Positive CoOp retains positive prompt learning in input space, but starts with a fixed negative prompt and learns it in feature space.\\
3) Positive CoOp requires YY times fewer training parameters and YY times fewer GPU hours than the SOTA method while training on COCO, and YY times fewer parameters and YY times fewer GPU hours while training on VOC2007. 


==> tables/cp_cr_cf.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c||c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{\% Labels}} & \multicolumn{7}{c||}{\textbf{COCO Dataset}} & \multicolumn{7}{c}{\textbf{VOC2007 Dataset}} \\ \cline{2-15} 
 & \textbf{CP} & \textbf{CR} & \textbf{CF1} & \textbf{OP} & \textbf{OR} & \textbf{OF1} & \textbf{mAP} & \textbf{CP} & \textbf{CR} & \textbf{CF1} & \textbf{OP} & \textbf{OR} & \textbf{OF1} & \textbf{mAP} \\ \hline
10\% & 73.4 & 77.9 & 75.1 & 74.8 & 82.2 & 78.3 & 81.1 &   82.5 & 90.3 & 85.2 & 81.0 & 92.5 & 86.4 & 92.5 \\ \hline
20\% & 75.6 & 78.6 & 76.9 & 77.8 & 82.8 & 80.3 & 83.1 &   85.39 & 89.6 & 87.2 & 86.9 & 91.3 & 89.0 & 93.5 \\ \hline
30\% & 75.0 & 80.1 & 77.1 & 77.0 & 83.9 & 80.3 & 83.8 &   84.3 & 91.7 & 87.4 & 85.9 & 92.8 & 89.2 & 94.0 \\ \hline
40\% & 76.3 & 80.2 & 78.0 & 78.4 & 83.9 & 81.0 & 84.4 &   82.8 & 92.46 & 86.9 & 83.0 & 94.2 & 88.2 & 94.3 \\ \hline
50\% & 77.2 & 80.6 & 78.4 & 78.5 & 84.2 & 81.3 & 85.0 &   86.6 & 91.6 & 88.7 & 88.2 & 92.7 & 90.4 & 94.6 \\ \hline
60\% & 77.5 & 80.6 & 78.7 & 78.8 & 84.3 & 81.5 & 85.1 &   85.2 & 93.1 & 88.4 & 84.6 & 94.2 & 89.1 & 94.6 \\ \hline
70\% & 77.5 & 80.7 & 78.9 & 79.1 & 84.4 & 81.7 & 85.2 &   84.5 & 93.4 & 88.4 & 84.9 & 94.7 & 89.5 & 94.9 \\ \hline
80\% & 77.9 & 80.9 & 79.1 & 79.1 & 84.6 & 81.8 & 85.6 &   85.9 & 92.1 & 88.6 & 88.7 & 92.6 & 90.6 & 94.9 \\ \hline
90\% & 78.0 & 81.1 & 79.2 & 79.2 & 84.8 & 81.9 & 85.7 &   85.0 & 93.3 & 88.7 & 86.6 & 94.4 & 90.3 & 95.2 \\ \hline
\end{tabular}
\caption{Performance on all metrics: per-class and overall average precisions (CP and OP), recalls (CR and OR), F1 scores (CF1 and OF1) and mAP for different ranges of limited labels (10\%-90\%) on the COCO \cite{coco} and VOC2007 \cite{pascal-voc} datasets}
\label{tab:cp_cr_cf}
\end{table*}


==> tables/linear_ablation.tex <==
\begin{table}[H]
% \scriptsize
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{\#Params} & \textbf{10\%} & \textbf{50\%} & \textbf{90\%} \\
\hline
\multirow{3}{*}{COCO} 
 & 1-MLP & 82k & 79.8 & 83.4 & 84.4 \\
 & 2-MLP & 134k & 80.4 & 84.1 & 84.8 \\
 & 3-MLP & 183k & 81.1 & 85.0 & 85.6 \\
\hline
\multirow{3}{*}{VOC 2007} 
 & 1-MLP & 20k & 90.8 & 94.0 & 94.7 \\
 & 2-MLP & 110k & 92.5 & 94.5 & 94.8 \\
 & 3-MLP & 168k & 92.7 & 94.7 & 95.2 \\
\hline
\end{tabular}
\caption{\textbf{Ablation on MLP depth}:  Performance and training parameter count for our MLP setup with varying number of layers. We find that increasing the number of layers consistently improves mAP across all ranges of limited labels. However, beyond three layers, we observe only marginal gains in performance}
\label{tab:linear_ablation}
\end{table}


==> tables/spatial_aggregation_ablation.tex <==
\begin{table}[H]
\centering
\begin{tabular}{l|ccc}
\hline
\textbf{Spatial Aggregation} & \textbf{10\%} & \textbf{50\%} & \textbf{90\%} \\ \hline
Multi-Headed Attention & 89.8& 91.4& 93.6\\ 
DualCoOp Aggregation & 91.3& 93.9& 94.9\\ 
\hline
Ours & 92.7 & 94.7 & 95.2 \\ \hline
\end{tabular}
\caption{\textbf{Comparing Spatial Aggregation Stratergies}: Comparison of our spatial aggregation methods with multi-headed attention in CLIP and DualCoOp's class-specific feature aggregation at different percentages of available labels on the VOC2007 \cite{pascal-voc} dataset. The results show that our aggregation strategy yields the best performance.}
\label{tab:spatial_aggregation}
\end{table}

==> tables/text_ablation.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{l|c|c|ccc}
\toprule
Dataset & Method & \# Params & 10\% & 50\% & 90\% \\
\midrule
\multirow{5}{*}{VOC2007 \cite{pascal-voc}} 
&DualCoOp \cite{dualcoop} & 0.3M  & 90.3 & 93.6 & 94.2 \\
&SCPNet \cite{scpnet} & - & 91.1 & 93.8 & 94.3 \\
&DualCoOp++ \cite{dualcoop++} & 0.4M & 92.7 & 94.3 & 94.9 \\
&Ours(1-MLP) & 20k&  90.1&  93.6& 94.2 \\
&DualCoOp-Positive & 152k&  91.4&  93.7& 94.3 \\
\midrule
\multirow{5}{*}{COCO  \cite{coco}} 
&DualCoOp \cite{dualcoop} & 1.3M & 78.7 & 82.5 & 83.1 \\
&SCPNet \cite{scpnet} & 3.4M & 79.1 & 83.8 & 84.2 \\
&TaI-DPT \cite{TaI-DPT} & 1.3M & 81.0 & 83.9 & 84.5 \\

&DualCoOp++ \cite{dualcoop++} & 1.5M & 81.4 & 84.4 & 85.1 \\
&Ours(1-MLP) & 152k&  78.4&  82.7& 83.6 \\
&DualCoOp-Positive & 681k &  78.9 & 82.9  & 84.0 \\


\bottomrule
\end{tabular}
\caption{We compare the SOTA MLR approaches with two variants proposed by us. Absence of a negative prompt improves DualCoOp's performance on both benchmarks, while even a simple baseline training a linear layer on top of a frozen visual encoder shows performance similar to past methods while using upto 18x fewer parameters.}
\label{tab:text ablation}
\end{table}
